nlfem: A flexible 2d Fem Code for Nonlocal Convection-Diffusion and Mechanics

In this work we present the mathematical foundation of an assembly code for finite element approximations of nonlocal models with compactly supported, weakly singular kernels. We demonstrate the code on a nonlocal diffusion model in various configurations and on a two-dimensional bond-based peridynamics model. The code nlfem is published under the MIT License and can be freely downloaded.

==> tables/parefficiency2.tex <==
\begin{longtable}[]{@{}ll@{}}
\toprule
Threads & Time\tabularnewline
\midrule
\endhead
1 & 2153\tabularnewline
2 & 1169\tabularnewline
4 & 583\tabularnewline
8 & 302\tabularnewline
16 & 166\tabularnewline
32 & 107\tabularnewline
64 & 80\tabularnewline
\bottomrule
\end{longtable}


==> tables/rates_kronos_0531_13-51-29.tex <==
\subsubsection{Setting}\label{setting}

\begin{longtable}[]{@{}ll@{}}
\toprule
Ansatz space & DG\tabularnewline
Right hand side & linearField\tabularnewline
\textbf{Kernel} &
\textbf{linearPrototypeMicroelasticField}\tabularnewline
Horizon \(\delta\) & 0.1\tabularnewline
Fractional constant \(s\)\tabularnewline
(Default -1) & -0.5\tabularnewline
\textbf{Intgr. remote pairs} & \textbf{retriangulate}\tabularnewline
With caps & True\tabularnewline
Quadrule outer element & 7\tabularnewline
Quadrule inner element & 16\tabularnewline
\textbf{Intgr. close pairs}\tabularnewline
(Relevant only if singular) & \textbf{retriangulate}\tabularnewline
Singular quad degree & 0\tabularnewline
\bottomrule
\end{longtable}

\subsubsection{Rates}\label{rates}

\begin{longtable}[]{@{}lllll@{}}
\toprule
h & dof & L2 Error & Rates & Time {[}s{]}\tabularnewline
\midrule
\endhead
1.00e-01 & 1.60e+01 & 6.64e-04 & 0.00e+00 & 1.42e-01\tabularnewline
5.00e-02 & 8.10e+01 & 1.86e-04 & 1.84e+00 & 3.11e+00\tabularnewline
2.50e-02 & 3.61e+02 & 4.96e-05 & 1.90e+00 & 4.81e+01\tabularnewline
1.25e-02 & 1.52e+03 & 1.25e-05 & 1.99e+00 & 6.89e+02\tabularnewline
6.25e-03 & 6.24e+03 & 2.92e-06 & 2.10e+00 & 1.04e+04\tabularnewline
\bottomrule
\end{longtable}

\newpage 

\subsubsection{Setting}\label{setting-1}

\begin{longtable}[]{@{}ll@{}}
\toprule
Ansatz space & CG\tabularnewline
Right hand side & linearField\tabularnewline
\textbf{Kernel} &
\textbf{linearPrototypeMicroelasticField}\tabularnewline
Horizon \(\delta\) & 0.1\tabularnewline
Fractional constant \(s\)\tabularnewline
(Default -1) & -0.5\tabularnewline
\textbf{Intgr. remote pairs} & \textbf{retriangulate}\tabularnewline
With caps & True\tabularnewline
Quadrule outer element & 7\tabularnewline
Quadrule inner element & 16\tabularnewline
\textbf{Intgr. close pairs}\tabularnewline
(Relevant only if singular) & \textbf{retriangulate}\tabularnewline
Singular quad degree & 0\tabularnewline
\bottomrule
\end{longtable}

\subsubsection{Rates}\label{rates-1}

\begin{longtable}[]{@{}lllll@{}}
\toprule
h & dof & L2 Error & Rates & Time {[}s{]}\tabularnewline
\midrule
\endhead
1.00e-01 & 1.60e+01 & 7.47e-04 & 0.00e+00 & 1.17e-01\tabularnewline
5.00e-02 & 8.10e+01 & 1.82e-04 & 2.04e+00 & 1.29e+01\tabularnewline
2.50e-02 & 3.61e+02 & 4.58e-05 & 1.99e+00 & 2.14e+01\tabularnewline
1.25e-02 & 1.52e+03 & 1.12e-05 & 2.04e+00 & 3.18e+02\tabularnewline
6.25e-03 & 6.24e+03 & 2.63e-06 & 2.09e+00 & 5.03e+03\tabularnewline
\bottomrule
\end{longtable}

\newpage 

